Kraken: Higher-order EM Side-Channel Attacks on DNNs in Near and Far Field

The multi-million dollar investment required for modern machine learning (ML) has made large ML models a prime target for theft. In response, the field of model stealing has emerged. Attacks based on physical side-channel information have shown that DNN model extraction is feasible, even on CUDA Cores in a GPU. For the first time, our work demonstrates parameter extraction on the specialized GPU's Tensor Core units, most commonly used GPU units nowadays due to their superior performance, via near-field physical side-channel attacks. Previous work targeted only the general-purpose CUDA Cores in the GPU, the functional units that have been part of the GPU since its inception. Our method is tailored to the GPU architecture to accurately estimate energy consumption and derive efficient attacks via Correlation Power Analysis (CPA). Furthermore, we provide an exploratory analysis of hyperparameter and weight leakage from LLMs in far field and demonstrate that the GPU's electromagnetic radiation leaks even 100 cm away through a glass obstacle.

==> tex/name.tex <==
\subsection{Far Field Parameter Extraction}\label{sec::app}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.75\columnwidth}
        \centering
        \includesvg[width=\linewidth]{cpa_results/key_rank_traceQ_row_0_slice8_w_8_zoom_1606_1610.eps}
        \caption{Key rank for the 8th weight in $\mathbf{W_q}$, reaching key rank 0.}
    \end{subfigure}%
    
    \begin{subfigure}{0.75\columnwidth}
        \centering
        \includesvg[width=\linewidth]{cpa_results/key_rank_traceK_row_0_slice8_w_8_zoom_1086_1087.eps}
        \caption{Key rank for the 8th weight in $\mathbf{W_k}$, reaching key rank 4.}
    \end{subfigure}

    \begin{subfigure}{0.75\columnwidth}
        \centering
        \includesvg[width=\linewidth]{cpa_results/key_rank_traceV_row_0_slice8_w_8_zoom_1755_1760.eps}
        \caption{Key rank for the 8th weight in $\mathbf{W_v}$, reaching key rank 11.}
    \end{subfigure}
    
    \caption{Key rankings for different weights in each projection matrix. The number of averaged traces used for CPA is 4000. Averaging is done for traces with the same inputs, with the total of 2 million traces before averaging. In principle, there is weight leakage in far field, but the practical use is limited for the attack.}
\end{figure}

==> tex/results.tex <==
\subsection{CPA results}\label{ssec::ff_cpa}
As a proof-of-concept, we demonstrate the extraction parameters in far-field, assuming we know the first 7 weights in the matrices $\mathbf{W_q}, \mathbf{W_k}, \mathbf{W_v}$, and we target the 8th weight, so we only have 5106 candidates for CPA.
By building the leakage models on the power consumption of individual warps, we can reach low key ranks for weights from $\mathbf{W}_q, \mathbf{W}_k, \mathbf{W}_v$ from 100 cm away from the GPU die through glass. We average 500 traces for each input, and we use 4000 different inputs, i.e., the number of collected traces is 2 million.

\lukasz{The X axis in the figures is unclear. Maybe key evolution rand would be useful.}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{cpa_results/corr_traceQ_7_rank_sub1_zoom_0_3300.eps}
        \caption{Full correlation trace for the 8th weight in $\mathbf{W_q}$.}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{cpa_results/corr_traceQ_7_rank_sub1_zoom_1600_1620.eps}
        \caption{Zoomed correlation trace for the 8th weight in $\mathbf{W_q}$ at samples 1600-1620 where the ranks goes to 1.}
    \end{subfigure}
    \caption{Correlation traces for the 8th weight in $\mathbf{W_q}$ from 100 cm away from the GPU die.}\label{fig::wq7}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{cpa_results/corr_trace_K_7_rank_sub5_zoom_0_3300.eps}
        \caption{Full correlation trace for the 8th weight in $\mathbf{W_k}$.}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{cpa_results/corr_trace_K_7_rank_sub5_zoom_1080_1090.eps}
        \caption{Zoomed correlation trace for the 8th weight in $\mathbf{W_k}$ at samples 1080-1090 where the ranks goes to 4.}
    \end{subfigure}
    \caption{Correlation traces for the 8th weight in $\mathbf{W_k}$ from 100 cm away from the GPU die.}\label{fig::wk7}
\end{figure*}

The results are shown for the 8th weight in each of the matrices $\mathbf{W_q}, \mathbf{W_k}, \mathbf{W_v}$ in \cref{fig::wq7,fig::wk7,fig::wv7}. In general, summing up the power consumptions related to the same weight in warp matrix-multiply instruction is a viable strategy. At 25 cm away from the die without glass in between, collecting only 1M traces with averaging already provides better results than 2M traces collected 100 cm away from the die with glass in between. 
Overall, we stil expect to get better results with more traces but our results already show the feasibility of this attack. Although attacking 44 bits is not infeasible, it is still not within our capabilities to mount attack of this scale. 

\lukasz{Some justification on not exploring 44 bits should be given here?}\peter{fixed}

\lukasz{Also, are 25cm much better? Would it make sense to add something about that? I think that one figure would be useful. }
\peter{added some text}

\begin{comment}
\subsection{Deep-learning based attack}
The deep learning based attack with the identity leakage model has shown inconsistent results when tested with different weights. While some weights can be recovered with 500k attack traces, some weights were not recovered even with 1 million attack traces. Perhaps, a Hamming-weight leakage model would work better but there are large class imbalances. Since in CPA we sum up the power consumptions of individual threads in a warp, the deep learning model would have to covert range of possible HW weights. Since the intermediates are \emph{float32}, each intermediate can contribute 32 to the total Hamming-weight. With multiple intermediates, such as 8 as in the CPA attack, the range of Hamming-weights can easily go into the hundreds. For instance, for 8 intermediates it is $8\times32=256$ classes. The major issue is the heavy imbalance present between the different Hamming-weights. The distribution of Hamming-weights has a large peak at 120-130 with long tails. To avoid overfitting, undersampling  could be used, but this potentially implies collecting a large training dataset in the order of tens of millions traces for a succesful attack.
\end{comment}
